Soft Syndrome Decoding of Quantum LDPC Codes for Joint Correction of Data and Syndrome Errors

Quantum errors are primarily detected and corrected using the measurement of syndrome information which itself is an unreliable step in practical error correction implementations. Typically, such faulty or noisy syndrome measurements are modeled as a binary measurement outcome flipped with some probability. However, the measured syndrome is in fact a discretized value of the continuous voltage or current values obtained in the physical implementation of the syndrome extraction. In this paper, we use this "soft" or analog information without the conventional discretization step to benefit the iterative decoders for decoding quantum low-density parity-check (QLDPC) codes. Syndrome-based iterative belief propagation decoders are modified to utilize the syndrome-soft information to successfully correct both data and syndrome errors simultaneously, without repeated measurements. We demonstrate the advantages of extracting the soft information from the syndrome in our improved decoders, not only in terms of comparison of thresholds and logical error rates for quasi-cyclic lifted-product QLDPC code families, but also for faster convergence of iterative decoders. In particular, the new BP decoder with noisy syndrome performs as good as the standard BP decoder under ideal syndrome.

==> figures/LP_FER_SyndTh_p05_Noisy_vs_D4.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=0,
xmax=0.7,
xlabel={$\text{Syndrome Noise }\sigma$},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymode=log,
ymin=0.001,
ymax=1,
yminorticks=true,
ylabel={Logical Error Rate at p = 0.05},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.2pt, mark size=2.0pt, mark=*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0	0.047812\\
0.1	0.049581\\
0.11	0.049581\\
0.12	0.049581\\
0.13	0.049581\\
0.14	0.049581\\
0.15	0.049581\\
0.16	0.049581\\
0.17	0.049581\\
0.18	0.049581\\
0.19	0.049581\\
0.2	0.049586\\
0.21	0.049719\\
0.22	0.05004\\
0.23	0.050398\\
0.24	0.051078\\
0.25	0.052874\\
0.26	0.056348\\
0.27	0.060972\\
0.28	0.070013\\
0.29	0.081873\\
0.3	0.095988\\
0.31	0.119804\\
0.32	0.14938\\
0.33	0.187825\\
0.34	0.229008\\
0.35	0.27439\\
0.36	0.330268\\
0.37	0.3915\\
0.38	0.4569\\
0.39	0.5169\\
0.4	0.5814\\
0.41	0.6396\\
0.42	0.6979\\
0.43	0.7531\\
0.44	0.7993\\
0.45	0.8386\\
0.46	0.8735\\
0.47	0.9084\\
0.48	0.9311\\
0.49	0.9521\\
0.5	0.963\\
0.51	0.9746\\
0.52	0.9845\\
0.53	0.9901\\
0.54	0.9925\\
0.55	0.9959\\
0.56	0.9968\\
0.57	0.9982\\
0.58	0.9987\\
0.59	0.9989\\
0.6	0.9994\\
0.61	0.9995\\
0.62	0.9998\\
0.63	0.9999\\
0.64	0.9999\\
0.65	0.9999\\
0.66	1\\
0.67	1\\
0.68	1\\
0.69	1\\
0.7	1\\
0.71	1\\
0.72	1\\
0.73	1\\
0.74	1\\
0.75	1\\
0.76	1\\
0.77	1\\
0.78	1\\
0.79	1\\
0.8	1\\
0.81	1\\
0.82	1\\
0.83	1\\
0.84	1\\
0.85	1\\
0.86	1\\
0.87	1\\
0.88	1\\
0.89	1\\
0.9	1\\
0.91	1\\
0.92	1\\
0.93	1\\
0.94	1\\
0.95	1\\
0.96	1\\
0.97	1\\
0.98	1\\
0.99	1\\
};
\addlegendentry{[[442,68,10]] Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark size=1.4pt, mark=square*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0	0.016665\\
0.1	0.015964\\
0.11	0.015964\\
0.12	0.015964\\
0.13	0.015964\\
0.14	0.015964\\
0.15	0.015964\\
0.16	0.015964\\
0.17	0.015964\\
0.18	0.015964\\
0.19	0.015964\\
0.2	0.016073\\
0.21	0.016231\\
0.22	0.016578\\
0.23	0.017451\\
0.24	0.019522\\
0.25	0.023554\\
0.26	0.029766\\
0.27	0.040069\\
0.28	0.057984\\
0.29	0.081096\\
0.3	0.112677\\
0.31	0.154769\\
0.32	0.206459\\
0.33	0.272246\\
0.34	0.341132\\
0.35	0.422316\\
0.36	0.501\\
0.37	0.572086\\
0.38	0.645271\\
0.39	0.711929\\
0.4	0.7755\\
0.41	0.8338\\
0.42	0.8778\\
0.43	0.9113\\
0.44	0.9374\\
0.45	0.96\\
0.46	0.9748\\
0.47	0.9847\\
0.48	0.9895\\
0.49	0.994\\
0.5	0.9964\\
0.51	0.9975\\
0.52	0.9991\\
0.53	0.9991\\
0.54	0.9997\\
0.55	1\\
0.56	1\\
0.57	1\\
0.58	1\\
0.59	1\\
0.6	1\\
0.61	1\\
0.62	1\\
0.63	1\\
0.64	1\\
0.65	1\\
0.66	1\\
0.67	1\\
0.68	1\\
0.69	1\\
0.7	1\\
0.71	1\\
0.72	1\\
0.73	1\\
0.74	1\\
0.75	1\\
0.76	1\\
0.77	1\\
0.78	1\\
0.79	1\\
0.8	1\\
0.81	1\\
0.82	1\\
0.83	1\\
0.84	1\\
0.85	1\\
0.86	1\\
0.87	1\\
0.88	1\\
0.89	1\\
0.9	1\\
0.91	1\\
0.92	1\\
0.93	1\\
0.94	1\\
0.95	1\\
0.96	1\\
0.97	1\\
0.98	1\\
0.99	1\\
};
\addlegendentry{[[714,100,16]] Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark size=3.5pt, mark=diamond*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0	0.004651\\
0.1	0.004526\\
0.11	0.004526\\
0.12	0.004526\\
0.13	0.004526\\
0.14	0.004526\\
0.15	0.004526\\
0.16	0.004526\\
0.17	0.004526\\
0.18	0.004526\\
0.19	0.00454\\
0.2	0.004587\\
0.21	0.004732\\
0.22	0.005191\\
0.23	0.006332\\
0.24	0.008529\\
0.25	0.012496\\
0.26	0.019915\\
0.27	0.032947\\
0.28	0.050937\\
0.29	0.078131\\
0.3	0.113307\\
0.31	0.164534\\
0.32	0.222711\\
0.33	0.2904\\
0.34	0.3741\\
0.35	0.4543\\
0.36	0.5419\\
0.37	0.619\\
0.38	0.6988\\
0.39	0.7662\\
0.4	0.8299\\
0.41	0.8855\\
0.42	0.9261\\
0.43	0.9537\\
0.44	0.9734\\
0.45	0.9836\\
0.46	0.9919\\
0.47	0.9969\\
0.48	0.9985\\
0.49	0.9993\\
0.5	0.9994\\
0.51	1\\
0.52	1\\
0.53	0.9999\\
0.54	1\\
0.55	1\\
0.56	1\\
0.57	1\\
0.58	1\\
0.59	1\\
0.6	1\\
0.61	1\\
0.62	1\\
0.63	1\\
0.64	1\\
0.65	1\\
0.66	1\\
0.67	1\\
0.68	1\\
0.69	1\\
0.7	1\\
0.71	1\\
0.72	1\\
0.73	1\\
0.74	1\\
0.75	1\\
0.76	1\\
0.77	1\\
0.78	1\\
0.79	1\\
0.8	1\\
0.81	1\\
0.82	1\\
0.83	1\\
0.84	1\\
0.85	1\\
0.86	1\\
0.87	1\\
0.88	1\\
0.89	1\\
0.9	1\\
0.91	1\\
0.92	1\\
0.93	1\\
0.94	1\\
0.95	1\\
0.96	1\\
0.97	1\\
0.98	1\\
0.99	1\\
};
\addlegendentry{[[1020,136,20]] Hard synd}

\addplot [color=blue, line width=1.2pt, mark size=2.0pt, mark=*, mark options={solid, fill=white, blue}]
  table[row sep=crcr]{%
0	0.047812\\
0.1	0.049581\\
0.11	0.049581\\
0.12	0.049581\\
0.13	0.049581\\
0.14	0.049581\\
0.15	0.049581\\
0.16	0.049581\\
0.17	0.049581\\
0.18	0.049586\\
0.19	0.049581\\
0.2	0.049719\\
0.21	0.049662\\
0.22	0.049801\\
0.23	0.049586\\
0.24	0.049586\\
0.25	0.049483\\
0.26	0.05004\\
0.27	0.050053\\
0.28	0.050186\\
0.29	0.050651\\
0.3	0.0516\\
0.31	0.053717\\
0.32	0.055188\\
0.33	0.058716\\
0.34	0.060783\\
0.35	0.067563\\
0.36	0.075821\\
0.37	0.083507\\
0.38	0.096544\\
0.39	0.1121\\
0.4	0.1327\\
0.41	0.1577\\
0.42	0.1855\\
0.43	0.2207\\
0.44	0.2578\\
0.45	0.3046\\
0.46	0.3524\\
0.47	0.4084\\
0.48	0.4672\\
0.49	0.5218\\
0.5	0.5777\\
0.51	0.6307\\
0.52	0.685\\
0.53	0.7327\\
0.54	0.7769\\
0.55	0.8153\\
0.56	0.8486\\
0.57	0.8786\\
0.58	0.8999\\
0.59	0.9227\\
0.6	0.939\\
0.61	0.9533\\
0.62	0.9633\\
0.63	0.9714\\
0.64	0.977\\
0.65	0.9826\\
0.66	0.9874\\
0.67	0.9917\\
0.68	0.9936\\
0.69	0.9957\\
0.7	0.9968\\
0.71	0.9975\\
0.72	0.9983\\
0.73	0.9987\\
0.74	0.9988\\
0.75	0.9992\\
0.76	0.9992\\
0.77	0.9994\\
0.78	0.9994\\
0.79	0.9993\\
0.8	0.9995\\
0.81	0.9996\\
0.82	0.9996\\
0.83	0.9997\\
0.84	0.9999\\
0.85	0.9999\\
0.86	0.9998\\
0.87	0.9999\\
0.88	1\\
0.89	1\\
0.9	1\\
0.91	1\\
0.92	1\\
0.93	1\\
0.94	1\\
0.95	1\\
0.96	1\\
0.97	1\\
0.98	1\\
0.99	1\\
};
\addlegendentry{[[442,68,10]] Soft synd}

\addplot [color=blue, line width=1.2pt, mark size=1.4pt, mark=square*, mark options={solid, fill=white, blue}]
  table[row sep=crcr]{%
0	0.016665\\
0.1	0.015964\\
0.11	0.015964\\
0.12	0.015966\\
0.13	0.015966\\
0.14	0.015964\\
0.15	0.016067\\
0.16	0.015966\\
0.17	0.016019\\
0.18	0.015877\\
0.19	0.016202\\
0.2	0.01617\\
0.21	0.016268\\
0.22	0.015966\\
0.23	0.015926\\
0.24	0.015933\\
0.25	0.016281\\
0.26	0.015966\\
0.27	0.016306\\
0.28	0.016306\\
0.29	0.01656\\
0.3	0.017322\\
0.31	0.018699\\
0.32	0.020716\\
0.33	0.022572\\
0.34	0.0256\\
0.35	0.030262\\
0.36	0.038921\\
0.37	0.050108\\
0.38	0.065355\\
0.39	0.083264\\
0.4	0.108802\\
0.41	0.141372\\
0.42	0.186063\\
0.43	0.238752\\
0.44	0.297141\\
0.45	0.362355\\
0.46	0.433057\\
0.47	0.507849\\
0.48	0.588141\\
0.49	0.654\\
0.5	0.7199\\
0.51	0.7753\\
0.52	0.8221\\
0.53	0.8687\\
0.54	0.9007\\
0.55	0.9253\\
0.56	0.9483\\
0.57	0.9626\\
0.58	0.9749\\
0.59	0.9824\\
0.6	0.9882\\
0.61	0.992\\
0.62	0.9939\\
0.63	0.9957\\
0.64	0.9975\\
0.65	0.9983\\
0.66	0.999\\
0.67	0.9992\\
0.68	0.9996\\
0.69	0.9998\\
0.7	0.9998\\
0.71	0.9999\\
0.72	0.9999\\
0.73	0.9999\\
0.74	0.9999\\
0.75	0.9999\\
0.76	1\\
0.77	1\\
0.78	1\\
0.79	1\\
0.8	1\\
0.81	1\\
0.82	1\\
0.83	1\\
0.84	1\\
0.85	1\\
0.86	1\\
0.87	1\\
0.88	1\\
0.89	1\\
0.9	1\\
0.91	1\\
0.92	1\\
0.93	1\\
0.94	1\\
0.95	1\\
0.96	1\\
0.97	1\\
0.98	1\\
0.99	1\\
};
\addlegendentry{[[714,100,16]] Soft synd}

\addplot [color=blue, line width=1.2pt, mark size=3.5pt, mark=diamond*, mark options={solid, fill=white, blue}]
  table[row sep=crcr]{%
0	0.004651\\
0.1	0.004526\\
0.11	0.004535\\
0.12	0.004526\\
0.13	0.0045\\
0.14	0.004525\\
0.15	0.004468\\
0.16	0.004468\\
0.17	0.00447\\
0.18	0.00447\\
0.19	0.004518\\
0.2	0.004404\\
0.21	0.004335\\
0.22	0.004383\\
0.23	0.004258\\
0.24	0.004255\\
0.25	0.004444\\
0.26	0.004526\\
0.27	0.004632\\
0.28	0.004964\\
0.29	0.005322\\
0.3	0.005846\\
0.31	0.006788\\
0.32	0.008722\\
0.33	0.011345\\
0.34	0.015929\\
0.35	0.021094\\
0.36	0.029563\\
0.37	0.042808\\
0.38	0.060555\\
0.39	0.088936\\
0.4	0.121457\\
0.41	0.1675\\
0.42	0.218706\\
0.43	0.285171\\
0.44	0.3581\\
0.45	0.4481\\
0.46	0.527\\
0.47	0.6117\\
0.48	0.6929\\
0.49	0.7651\\
0.5	0.8254\\
0.51	0.874\\
0.52	0.9155\\
0.53	0.9421\\
0.54	0.9641\\
0.55	0.9786\\
0.56	0.9863\\
0.57	0.9921\\
0.58	0.9949\\
0.59	0.9968\\
0.6	0.9978\\
0.61	0.9988\\
0.62	0.9993\\
0.63	0.9998\\
0.64	0.9999\\
0.65	1\\
0.66	1\\
0.67	1\\
0.68	1\\
0.69	1\\
0.7	1\\
0.71	1\\
0.72	1\\
0.73	1\\
0.74	1\\
0.75	1\\
0.76	1\\
0.77	1\\
0.78	1\\
0.79	1\\
0.8	1\\
0.81	1\\
0.82	1\\
0.83	1\\
0.84	1\\
0.85	1\\
0.86	1\\
0.87	1\\
0.88	1\\
0.89	1\\
0.9	1\\
0.91	1\\
0.92	1\\
0.93	1\\
0.94	1\\
0.95	1\\
0.96	1\\
0.97	1\\
0.98	1\\
0.99	1\\
};
\addlegendentry{[[1020,136,20]] Soft synd}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> figures/LP_FER_threshold_025_Noisy_vs_D4_vs_Perfect_cutoff10.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=0.02,
xmax=0.1,
xlabel={Depolarizing Probability $(p)$},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymode=log,
ymin=1e-05,
ymax=1,
yminorticks=true,
ylabel={Logical Error Rate},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.2pt, mark=*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	0.002744\\
0.03	0.006423\\
0.04	0.018968\\
0.05	0.052874\\
0.06	0.122276\\
0.07	0.254349\\
0.08	0.4435\\
0.09	0.651235\\
0.1	0.8154\\
};
\addlegendentry{$[[442,68,10]]$ Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark=square*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	0.006276\\
0.03	0.008508\\
0.04	0.012751\\
0.05	0.023554\\
0.06	0.055844\\
0.07	0.144157\\
0.08	0.315268\\
0.09	0.5586\\
0.1	0.7912\\
};
\addlegendentry{$[[714,100,16]]$ Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark=diamond*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	0.011452\\
0.03	0.011261\\
0.04	0.00993\\
0.05	0.012496\\
0.06	0.0245\\
0.07	0.063243\\
0.08	0.194922\\
0.09	0.461661\\
0.1	0.7609\\
};
\addlegendentry{$[[1020,136,20]]$ Hard synd}

\addplot [color=blue, line width=1.2pt, mark=*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	0.000488\\
0.03	0.003778\\
0.04	0.015489\\
0.05	0.049569\\
0.06	0.118576\\
0.07	0.25165\\
0.08	0.4415\\
0.09	0.650535\\
0.1	0.814\\
};
\addlegendentry{$[[442,68,10]]$ Soft synd}

\addplot [color=blue, line width=1.2pt, mark=square*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	0.000183\\
0.03	0.001094\\
0.04	0.004882\\
0.05	0.016509\\
0.06	0.049227\\
0.07	0.137659\\
0.08	0.311269\\
0.09	0.5549\\
0.1	0.7902\\
};
\addlegendentry{$[[714,100,16]]$ Soft synd}

\addplot [color=blue, line width=1.2pt, mark=diamond*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	9.6e-05\\
0.03	0.000372\\
0.04	0.001322\\
0.05	0.004559\\
0.06	0.016407\\
0.07	0.05506\\
0.08	0.185726\\
0.09	0.455463\\
0.1	0.7598\\
};
\addlegendentry{$[[1020,136,20]]$ Soft synd}

\addplot [color=black, dashed, line width=1.2pt, mark=*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	0.000481\\
0.03	0.003468\\
0.04	0.015939\\
0.05	0.047812\\
0.06	0.12293\\
0.07	0.245375\\
0.08	0.437756\\
0.09	0.640172\\
0.1	0.8119\\
};
\addlegendentry{$[[442,68,10]]$ Perfect synd}

\addplot [color=black, dashed, line width=1.2pt, mark=square*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	0.000181\\
0.03	0.001209\\
0.04	0.004631\\
0.05	0.016665\\
0.06	0.047794\\
0.07	0.125362\\
0.08	0.305078\\
0.09	0.5567\\
0.1	0.7963\\
};
\addlegendentry{$[[714,100,16]]$ Perfect synd}

\addplot [color=black, dashed, line width=1.2pt, mark=diamond*, mark options={solid, fill=white}]
  table[row sep=crcr]{%
0.02	5.4e-05\\
0.03	0.00031\\
0.04	0.001175\\
0.05	0.004651\\
0.06	0.016772\\
0.07	0.057587\\
0.08	0.1878\\
0.09	0.4481\\
0.1	0.760324\\
};
\addlegendentry{$[[1020,136,20]]$ Perfect synd}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\end{axis}
\end{tikzpicture}%

==> figures/LP_Tanner_AvgNumIter_vs_p_Perfect_03_Hard_Soft.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=0.02,
xmax=0.1,
xlabel={Depolarizing Probability (p)},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymode=log,
ymin=4.584637,
ymax=149.230194,
yminorticks=true,
ylabel={Avg Number of Iterations},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.2pt, mark=*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0.02	39.347019\\
0.03	41.903938\\
0.04	43.889328\\
0.05	46.94405\\
0.06	51.675728\\
0.07	61.193165\\
0.08	77.272652\\
0.09	109.422997\\
0.1	149.230194\\
};
\addlegendentry{Hard synd}

\addplot [color=blue, line width=1.2pt, mark=square*, mark options={solid, fill=white, blue}]
  table[row sep=crcr]{%
0.02	6.902517\\
0.03	9.317492\\
0.04	12.468417\\
0.05	16.858681\\
0.06	22.623306\\
0.07	33.326439\\
0.08	54.310215\\
0.09	92.708298\\
0.1	140.783203\\
};
\addlegendentry{Soft synd}

\addplot [color=black, dashed, line width=1.2pt, mark=diamond*, mark options={solid, fill=white, black}]
  table[row sep=crcr]{%
0.02	4.584637\\
0.03	6.709046\\
0.04	9.581033\\
0.05	13.524993\\
0.06	19.351219\\
0.07	29.616133\\
0.08	50.653774\\
0.09	89.602898\\
0.1	138.883301\\
};
\addlegendentry{Perfect synd}

\end{axis}
\end{tikzpicture}%

==> figures/LP_Threshold_FER_vs_p_Hard_vs_Perfect_10_16_24.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=0.1,
xmax=0.11,
xticklabels={,0.1,,0.102,,0.104,,0.106,,0.108,,0.11,},
xlabel={Depolarizing $(p)$},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
%ymode=log,
ymin=0.73195,
ymax=0.95675,
%yminorticks=true,
ylabel={Logical Error Rate},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.2pt, mark=*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0.1	0.82515\\
0.102	0.85785\\
0.104	0.87605\\
0.106	0.8975\\
0.108	0.90945\\
0.11	0.9285\\
};
\addlegendentry{[[442,68,10]] Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark=square*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0.1	0.81175\\
0.102	0.8445\\
0.104	0.875912\\
0.106	0.89805\\
0.108	0.9195\\
0.11	0.93735\\
};
\addlegendentry{[[714,100,16]] Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark=diamond*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0.1	0.7815\\
0.102	0.8296\\
0.104	0.8725\\
0.106	0.9049\\
0.108	0.930503\\
0.11	0.95675\\
};
\addlegendentry{[[1428,184,24]] Hard synd}

\addplot [color=black, dashed, line width=1.2pt, mark=*, mark options={solid, fill=white, black}]
  table[row sep=crcr]{%
0.1	0.8145\\
0.102	0.8379\\
0.104	0.8618\\
0.106	0.8845\\
0.108	0.9064\\
0.11	0.92165\\
};
\addlegendentry{[[442,68,10]] Perfect synd}

\addplot [color=black, dashed, line width=1.2pt, mark=square*, mark options={solid, fill=white, black}]
  table[row sep=crcr]{%
0.1	0.7915\\
0.102	0.8238\\
0.104	0.858657\\
0.106	0.88725\\
0.108	0.9075\\
0.11	0.92865\\
};
\addlegendentry{[[714,100,16]] Perfect synd}

\addplot [color=black, dashed, line width=1.2pt, mark=diamond*, mark options={solid, fill=white, black}]
  table[row sep=crcr]{%
0.1	0.73195\\
0.102	0.79395\\
0.104	0.84305\\
0.106	0.88515\\
0.108	0.91745\\
0.11	0.94535\\
};
\addlegendentry{[[1428,184,24]] Perfect synd}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\node[below right, align=left, draw=black]
at (rel axis cs:0.511,0.13) {0.106};
\node[below right, align=left, draw=black]
at (rel axis cs:0.375,0.134) {$\text{\textless{} 0.105}$};
\end{axis}
\end{tikzpicture}%

==> figures/LP_Threshold_FER_vs_p_Hard_vs_Soft_10_16_24.tex <==
% This file was created by matlab2tikz.
%
%The latest updates can be retrieved from
%  http://www.mathworks.com/matlabcentral/fileexchange/22022-matlab2tikz-matlab2tikz
%where you can also make suggestions and rate matlab2tikz.
%
\begin{tikzpicture}

\begin{axis}[%
width=4.521in,
height=3.566in,
at={(0.758in,0.481in)},
scale only axis,
separate axis lines,
every outer x axis line/.append style={black},
every x tick label/.append style={font=\color{black}},
every x tick/.append style={black},
xmin=0.1,
xmax=0.11,
xlabel={Depolarizing Probability (p)},
every outer y axis line/.append style={black},
every y tick label/.append style={font=\color{black}},
every y tick/.append style={black},
ymode=log,
ymin=0.73985,
ymax=0.95675,
yminorticks=true,
ylabel={Logical Error Rate},
axis background/.style={fill=white},
xmajorgrids,
ymajorgrids,
yminorgrids,
legend style={at={(0.97,0.03)}, anchor=south east, legend cell align=left, align=left, draw=white!15!black}
]
\addplot [color=red, dashdotted, line width=1.2pt, mark=*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0.1	0.82515\\
0.102	0.85785\\
0.104	0.87605\\
0.106	0.8975\\
0.108	0.90945\\
0.11	0.9285\\
};
\addlegendentry{[[442,68,10]] Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark=square*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0.1	0.81175\\
0.102	0.8445\\
0.104	0.875912\\
0.106	0.89805\\
0.108	0.9195\\
0.11	0.93735\\
};
\addlegendentry{[[714,100,16]] Hard synd}

\addplot [color=red, dashdotted, line width=1.2pt, mark=diamond*, mark options={solid, fill=white, red}]
  table[row sep=crcr]{%
0.1	0.7815\\
0.102	0.8296\\
0.104	0.8725\\
0.106	0.9049\\
0.108	0.930503\\
0.11	0.95675\\
};
\addlegendentry{[[1428,184,24]] Hard synd}

\addplot [color=blue, line width=1.2pt, mark=*, mark options={solid, fill=white, blue}]
  table[row sep=crcr]{%
0.1	0.8145\\
0.102	0.84985\\
0.104	0.8708\\
0.106	0.8915\\
0.108	0.9049\\
0.11	0.92525\\
};
\addlegendentry{[[442,68,10]] Soft synd}

\addplot [color=blue, line width=1.2pt, mark=square*, mark options={solid, fill=white, blue}]
  table[row sep=crcr]{%
0.1	0.79385\\
0.102	0.82835\\
0.104	0.863714\\
0.106	0.88665\\
0.108	0.91295\\
0.11	0.9311\\
};
\addlegendentry{[[714,100,16]] Soft synd}

\addplot [color=blue, line width=1.2pt, mark=diamond*, mark options={solid, fill=white, blue}]
  table[row sep=crcr]{%
0.1	0.73985\\
0.102	0.7955\\
0.104	0.8477\\
0.106	0.88765\\
0.108	0.918754\\
0.11	0.9477\\
};
\addlegendentry{[[1428,184,24]] Soft synd}

\end{axis}

\begin{axis}[%
width=5.833in,
height=4.375in,
at={(0in,0in)},
scale only axis,
xmin=0,
xmax=1,
ymin=0,
ymax=1,
axis line style={draw=none},
ticks=none,
axis x line*=bottom,
axis y line*=left,
legend style={legend cell align=left, align=left, draw=white!15!black}
]
\node[below right, align=left, draw=black]
at (rel axis cs:0.511,0.13) {0.106};
\node[below right, align=left, draw=black]
at (rel axis cs:0.375,0.134) {$\text{\textless{} 0.105}$};
\end{axis}
\end{tikzpicture}%
